A Recommender System Based on a Double Feature Allocation Model

A collaborative filtering recommender system predicts user preferences by discovering common features among users and items. We implement such inference using a Bayesian double feature allocation model, that is, a model for random pairs of subsets. We use an Indian buffet process (IBP) to link users and items to features. Here a feature is a subset of users and a matching subset of items. By training feature-specific rating effects, we predict ratings. We use MovieLens Data to demonstrate posterior inference in the model and prediction of user preferences for unseen items compared to items they have previously rated. Part of the implementation is a novel semi-consensus Monte Carlo method to accomodate large numbers of users and items, as is typical for related applications. The proposed approach implements parallel posterior sampling in multiple shards of users while sharing item-related global parameters across shards.

==> abstract3.tex <==
A collaborative filtering recommender system predicts
user preferences by discovering
\bch common features among users \ech
and items. \cut % In this work
We implement such inference using a
Bayesian double feature allocation model, that is, a model for random
pairs of subsets. We use an Indian buffet
process (IBP) to link users and items to features.
Here a feature is a subset of users and a matching subset of items.
By training feature-specific rating effects, we predict ratings.
We use MovieLens Data to demonstrate posterior inference
\bch in \ech the model
and prediction of user preferences for unseen items compared to
items they have previously rated.

Part of the implementation is a \bch novel \ech
semi-consensus Monte Carlo method to
accomodate large numbers of users and items, as is typical for related
applications. The proposed approach implements parallel posterior
sampling in multiple shards of users while sharing item-related global
parameters across shards.


==> intro3.tex <==
\section{Introduction}
\label{sec:intro}
Collaborative Filtering is a recommender system approach to predict
personalized user preference for products (i.e, ratings, rankings) by
discovering similarity patterns among users and items, and \bch
providing \ech recommendations accordingly (\cite{itembased},
\cite{CFRS}, \cite{ACF}). It has been widely adopted by e-commerce
websites and online streaming services. The Netflix Prize since 2006
has encouraged more progress in this field.

The Netflix data (\cite{LDA-like}, \cite{ACF}, \cite{VCF1},
\cite{VCF2}) is
\bch a widely used \ech
dataset for collaborative
filtering research. It is a sparse matrix with 463435 users as rows,
17769 items (movies) as columns and 56.9 million interactions
(ratings) between them in 1999 to 2005 as entries. On average a movie
has 5600 ratings and a user rates 208 movies (\cite{ACF}). Thus the
density of the matrix is as low as 0.69\% (\cite{VCF2}).

\bch Collaborative filtering methods have \ech progressed from naive
nearest neighbor methods, to well-adopted matrix factorization
\bch methods, to
probabilistic Bayesian models with latent factors and, \bch
more recently, \ech to generative models.


Nearest neighbour methods (\cite{CFRS}, \cite{ACF}) \rd are intuitively appealing \bk. The
\bch idea is that
the rating $r_{ui}$ of user $u$ for item $i$ is likely to be close to
the ratings $r_{u'i}$ of similar users $u'$ for the same item, or, by
an equivalent argument, it is likely to be close to the ratings $r_{ui'}$
of similar items $i'$ by the same user $u$. \ech
The key here is to measure the similarity \bch of \ech users (or
items). The simplest measure uses the correlation coefficient.

\bch Using a similarity measure, \ech we can identify the $k$ 
items \bch that are most similar to $i$ \ech rated by $u$.
\bch Denote the set of such items by  $S^k(i;u)$ and the method predicts
$r_{ui}$ using a weighted average of the ratings
of items in $S^k(i;u)$ that are rated by user $u$, 
%\begin{equation}
%    \hat{r_{ui}}=b_{ui} + \frac{\sum_{j\in S^k(i;u)}s_{ij}(r_{uj}-b_{uj})}{\sum_{ j\in S^k(i;u)}s_{ij}},
%  \end{equation}
using weights proportional to the respective similarlities, \ech
i.e, the more similar the neighbour is, the more weight it gets.

%There are many versions of nearest %neightbours by twisting $b_{ui}$ or %$s_{ij}$, but they share the same %ideas and thus the same pros and %cons. They are simple models with %easy explanations. But when the %scale of users and items increases, %calculating pairwise similarity %becomes very inefficient. Even %worse, the similarity is ill defined %in the sparse case.  Say one user %has only watched 3 movies, from user %perspective, it is arbitrary to %assume he/she is similar to those %who watched 100 movies but have the %same ratings to these 3 movies. From %an item perspective, it is %meaningless to compare future movies %based on its similarity to only 3 %movies. 



\bch Assume now that ratings are metric. \ech
Matrix Factorization is one of the most popular methods in
collaborative filtering. The $m\times n$ rating matrix with $m$ users
and $n$ movies can be seen as the inner product of the a $k\times m$
matrix $P$ and $k \times n$ matrix $Q$, i.e, $R=P^TQ$.
\bch Here, \ech
$k$ is the \bch number \ech
of latent factors $z$, for example, movie genres. Then
\bch the $P$ matrix can be interpreted as representing the preferences 
of users for the \ech $k$ genres and \bch the $Q$ matrix
can be interpreted as a classification of the movies relative to \ech
these genres.
\bch The rating $r_{ui}$ for a specific movie and user then becomes
$r_{ui} = P_u^T Q_i$, using $P_u$ and $Q_i$ to denote the
corresponding row and column of $P$ and $Q$, respectively. \ech
\mynote{trying to use consistent notation --  later we used $P_u$ for
  the $u$-th row etc.. -- was $p_u$}

\bch The problem then is \ech
to find \bch preferences \ech $P$ and $Q$ \bch to best predict
observed ratings $r$ by $\rhat = p^Tq$,  while controlling \ech
% predicted rating $p^Tq$ is close to $r$, and we want control
the number of the latent
factors (the rank of $P$ and $Q$). Thus the objective is
\begin{equation*}
  min_{\rd Q,P}\sum_{u,i}(r_{ui}-p_{\rd u}^Tq_{\rd i})^2+
        \lambda(||q_i||^2+||p_{\rd u}||^2).
\end{equation*}
\mynote{Q: is the regularization $\lambda(||q_i||^2+||p_{\rd u}||^2$
  really inside the double sum over $i,u$? That sum would seem to
  include then $||q_i||$ as often as the number of users that rate
  item $i$, and similar for $||p_u||$??}
\bch The \ech parameter $\lambda$ is determined by cross
validation. Minimization is performed by stochastic gradient
descent. A popular one is performed by \cite{funk2006MF} and
\cite{Paterek2007MF}. %, iterate until convergence, 
%\begin{align}
%   & e_{ui} =r_{ui}-\hat{r_{ui}}\\
%   & q_i \xleftarrow[]{} q_i+\gamma (e_{ui}p_u-\lambda q_i)\\
%   & p_u \xleftarrow[]{} p_u+ \gamma (e_{ui}q_i-\lambda p_u)
%\end{align}
  
%Note that baseline predictors can be added to the error part of the objective function $\sum_{u,i}(r_{ui}-b_u-b_i-p^Tq)^2$. 
%Mild twists such as time varying factors $t_{ui}$ can be added into the baseline predictor as well (\cite{ACF}), such as $b_{ui}=\mu+b_u(t_{ui})+b_i(t_{ui})$, where the user or item's baseline preference is a function of time. 


Other similar methods include SVD++ (\cite{2says17}), where another set of latent factors $y_i$ are added to the model to characterize a user by what item they have already rated. 
%\begin{equation}
%    \hat{r_{ui}}=\mu+ b_i+b_u + (p_u+|R(u)|^{-\frac{1}{2}}\sum_{j \in R(u)}y_j)^Tq_i
%\end{equation}
%$R(u)$ is the set that contains all the items user $u$ has rated. Stochastic gradient descent can be updated as
%\begin{align}
%  & e_{ui} =r_{ui}-\hat{r_{ui}}\\
%   & b_{u} \xleftarrow{} b_{u}+\gamma(e_{ui}-\lambda b_u)\\
%  &  b_{i} \xleftarrow{} b_{i}+\gamma(e_{ui}-\lambda b_i)\\
%   & q_i \xleftarrow[]{} q_i+\gamma (e_{ui}(p_u+|R(u)|^{-\frac{1}{2}}\sum_{j \in R(u)}y_j))-\lambda q_i)\\
%   & p_u \xleftarrow{} p_u+ \gamma (e_{ui}q_i-\lambda p_u) \\
%   &\forall j\in R(u),\quad y_j\xleftarrow[]{} y_j +\gamma (e_{ui}|R(u)|^{-\frac{1}{2}}q_i-\lambda y_j)
%\end{align}

Matrix factorization captures the latent pattern in users and items. A convenient stochastic gradient descent made it a winner of the
Netflix prize.
\bch An additional advantage is the ease of \ech
incorporating temporal dynamics.
However, the point estimation of the prediction comes without an uncertainty measure and thus cannot serve a more complicated
goal of filtering and understanding user behavior, one of the reasons why
we introduce probabilistic models in the next section.



\rd \section{Probabilistic Models}
\subsection{Probabilistic Matrix Factorization} \bk
Probabilistic Matrix Factorization (\cite{PMF}) interprets Matrix
Factorization \bch from \ech a probabilistic perspective. They \bch
show \ech that
minimizing the sum of square errors
\cut % of matrix factorization objective
while penalizing their Frobenius norm is equivalent to maximizing the
log posterior in a probabilistic model with spherical Gaussian
priors. 

\bch As before, define $R=[r_{ui}]$ as the $(m \times n)$ rating
matrix, and $P$ and $Q$ are $(k\times m)$ and $(k\times n)$ \ech
the low rank latent feature-user and feature-item matrices.
\bch As before let $p_u$ and $q_i$ denote $i-$th row and $j-$th column
respectively, and \rd let $N(x|m,V)$ denote a normal p.d.f for random variable $x$ with moments $m$ and $V$. \ech
A
probabilistic model with Gaussian observation noise is defined
as \rd \begin{equation*} 
  p(R \mid P,Q,\sigma^2)=
  \prod^m_{\rd u=1}\prod^n_{\rd
    i=1}[N(r_{ui}|p_u^Tq_i,\sigma^2)]^{I_{\rd ui}}.
  \end{equation*} \bk
\mynote{Q: please synchronize notation with before.
  We have already introduced $u=1,\ldots,n$ for users and
  $i=1,\ldots,m$ for items.}
$I_{\rd ui}$ equals to $1$ if user $u$ has rated movie $\rd i$ and
equals to $0$ otherwise.
\bch The model is completed with \ech
zero-mean spherical Gaussian priors on $P$ and $Q$:
\rd 
\begin{equation*}
    p(P \mid \sigma_P^2)=\prod^m_{u=1} N(p_u \mid
    0,\sigma_P^2I),\quad p(Q \mid \sigma_Q^2)=
    \prod_{i=1}^n N(q_i \mid 0,\sigma_Q^2I) 
  \end{equation*}
  \bk
\mynote{Since we use $P$ for the matrix, maybe use $p(\cdot)$ for
  generic probabilities? instead of $P(\cdot)$?}
%Then the log posterior distribution over the user and movie is given by
%\begin{align}
%\begin{split}
%    \log p(P,Q|R,\sigma^2,\sigma_P^2,\sigma_Q^2)= &-\frac{1}{2\sigma^2}\sum_{i=1}^N\sum_{j=1}^MI_{ij}(R_{ij}-P_i^TQ_j)^2-\frac{1}{2\sigma_P^2}\sum_{i=1}^NP_i^TP_i-\frac{1}{2\sigma_Q^2}\sum_{j=1}^MQ_j^TQ_j\\
%    &-\frac{1}{2}((\sum_{i=1}^N\sum_{j=1}^M I_{ij})\log \sigma^2+ND\log \sigma_P^2 +MD \log \sigma_Q^2 )+Constant
%\end{split}
%\end{align}
Maximizing $\log p(P,Q|R,\sigma^2,\sigma_P^2,\sigma_Q^2)$
\bch in this model \ech is
equivalent to minimizing the sum of squares error with quadratic
regularization 
\begin{equation*}
    E=\frac{1}{2}\sum_{u=1}^m\sum_{i=1}^nI_{ui}(r_{ui}-p_u^Tq_i)^2+\frac{\lambda_P}{2}\sum_{u=1}^m ||p_u||^2_{Fro}+\frac{\lambda_Q}{2}\sum_{i=1}^n ||q_i||^2_{Fro},
\end{equation*}
where $\lambda_P=\frac{\sigma^2}{\sigma_P^2}$, $\lambda_Q=\frac{\sigma^2}{\sigma_Q^2}$.

A minibatch gradient descent is used to find the optimal $P$ and
$Q$. \bch The optimization defines \ech an extension of the classic SVD
model, where the
\bch modified SVD is defined seen as the MAP estimate, \ech
and the classic SVD is a special case where prior variance goes to infinity.  

%To guarantee the predicted value is within the valid rating range, we can pass a non-linear function $g(x)=\frac{1}{1+exp(-x)}$ through the predicted mean,
%\begin{equation*}
%    P(R|P,Q,\sigma^2)=\prod_{i=1}^J\prod_{j=1}^M [N(R_{ij}|g(U_i^TV_j),\sigma^2)]^{I_{ij}}.
%\end{equation*}
\rd
\cite{PMF} also discussed other constraints to be allowed onto the model. For all proposed models proposed, instead of adopting a full Bayesian approach and leading to a MCMC posterior simulation, the authors used stochastic gradient descent. This approach limits meaningful posterior inference for hyperparameters and uncertainty quantification of the MAP, but on the other hand has vastly decreased the computational cost.  \bk

\rd \subsection{Latent Dirichlet Allocation (LDA)-Like Model}\bk
\mynote{Q: please synchronize notation with before.
  We have already introduced $u=1,\ldots,n$ for users and
  $i=1,\ldots,m$ for items.}
User Rating Profile model (URP) proposed by Benjamin Marlin
(\cite{LDA-like}) represents each user as a mixture as a user
attitudes, and the mixture proportions are distributed according to a
Dirichlet random variable.

\mynote{Q: in this par, please change $U \leftrightarrow u$ \&
  $Y \leftrightarrow i$, to match the earlier notation, lest it's
  really consufing for any reader}
\cut %Define $\rd u$ as user index, $Y$ as item index,
For any user \bch $u$ we introduce a set of latent item-specific
attitudes
$Z_{ui}$. Here $Z_{ui}$ is a user attitude that determines the rating
of $i$.
Next, let $\beta_{viz} = P(r_{ui}=v \mid Z_{ui}=z)$ denote
item-specific rating probabilities.
Like in the Latent Dirichlet
Allocation (LDA) model, $\theta_u$ is a Dirichlet random variable with
parameter $\alpha$, and $p(Z=z)=\th_{uz}$. \ech

A user profile is thus $r_u=[r_{u1}, \ldots, r_{u,n}]$
\bch with a sampling model
$p(r_u \mid Z_{u}, \beta)$ determined by the described hierarchical
model. \ech
However, the posterior distribution for $\theta$ and $Z_u$ is
intractable. \bch It can be written as \ech
$$
  p(\theta_u, Z_u \mid r_u,\alpha,\beta) =
    \frac{p(\theta_u, Z_u, r_u \mid \alpha,\beta)}
    {p(r_u \mid \alpha,\beta)},
$$
\bch using the joint distribution of $(\th_u,Z_u,r_u)$ in the
numerator and 
\begin{multline}
p(r_u \mid \alpha,\beta) = \int_\theta
   dp(\theta_u \mid \alpha)
   \prod_{i=1}^n
   \sum_{z=1}^kp(Z_{ui}=z \mid \theta_u)
   p(r_{ui} \mid Z_{ui},\beta) = \\
   = \int \prod_i \left(    \sum_{z=1}^k \th_{uz} \beta_{r_{ui}iz} \right)\,
   dp(\theta_u \mid \alpha)
   \nonumber
 \end{multline}
\ech

They use a variational inference algorithm similar to LDA to approximate posterior inference. %A fully factored variational distribution $q$ is defined below.
Let $q(\theta|\gamma^u)$ denote a Dirichlet distribution with parameter $\gamma_z^u$ and $q(Z_y|\phi_y^u)$  be a multinomial distribution with parameters $\phi_{zy}^u$.  We use the variational distribution 
\begin{equation}
    p(\theta,z|\alpha,\beta,r_u)\approx q(\theta,z|\gamma^u,\phi^u)=q(\theta|\gamma^u)\prod_{y=1}^n q(Z_y=z_y|\phi_y^u)
\end{equation}


\rd  The updating steps of the Variational Bayes algorithm are similar to LDA. With an approximate of posterior distribution, instead of a point estimation, of the prediction, we can achieve multiple goals: MAP estimation, expected rating, median rating, etc and perform some uncertainty quantification of the prediction. \rd However, the URP model tends to overfit as the authors report. but in large scale applications, when it is impractical to refit the model every time a rating becomes available, URP outperforms traditional methods in prediction and speed.

\rd \subsection{Bayesian Mallows Model} \bk
Another string of papers on probabilistic models
\bch build on \ech Bayesian Mallows
Model (\cite{MM1}, \cite{MM2}, \cite{MM3}). Different from other
models, Mallows model \bch treats the response variables as ordinal
rankings. 
% uses rankings as the response variable.
For example, \ech \cite{MM1} work with the ranking of a user's rating
on n items, $r_u=\{r_{u1},r_{u2}, \ldots, r_{un}\}$, $u=1,2,3, \ldots, m$.
Mallows model is a \bch probability \ech model on the space $P_n$ of
permutations of $n$ items.

\rd A basic model uses a latent consensus ranking $\rho \in P_n$ to define, 
\begin{equation}
  P(r_{\rd u}=r \mid \alpha,\rho) {\rd \propto}
    % \frac{1}{Z_n(\alpha,\rho)
  \exp\left(-\frac{\alpha}{n}\, d(r,\rho) \right)
  \label{eq:mallows}
\end{equation}
\mynote{was $\propto 1/exp(-.. d(r,\rho))$ -- but that would be weird,
  putting more prob mass far away from $\rho$? \rd this is correct now \bk}  
where $\alpha$ is a scale parameter and
$d(r,\rho)=\sum_{i=1}^n|r_i-\rho_i|$ is a distance between $r$ and $\rho$.
\bch The normalizing constant 
$Z_n(\alpha,\rho)$ in \eqref{eq:mallows} 
is usually not analytically tractable. 
\cite{MM3}, for example, use instead importance sampling and
Metropolis-Hastings posterior simulation schemes. \ech

In a more complicated scenario where users are not homogeneous, $m$ users are arranged into $C$ clusters; each cluster has its own common consensus $\rho_c$. \rd Latent cluster membership indicator $z_u$ assign user $u$ to cluster $z_u$. The model is then
\begin{equation*}
     P(r_1,\ldots,r_m|\{\alpha_c,\rho_c\}_{\{c=1,,,C\}},z_1,\ldots,z_m)=\prod_{u=1}^m [Z_n(\alpha_{z_u})]^{-1}\exp(-\frac{\alpha_{z_u}}{n}d(r_u,\rho_{z_u})).
\end{equation*}
\bk
with exponential priors on $\alpha$, uniform prior on $\rho$, and a dirichlet prior on $\tau$.
%with priors
%\begin{align}
%& \pi(\alpha_1,,,\alpha_C|\lambda)=\lambda^C exp(-\lambda \sum_{c=1}^C\alpha_c) \quad \text{(exponential)}\\
%& \pi(\rho_1,,,,\rho_C)=n!^{-C} \quad \text{(uniform)}\\
%& p(z_1,,,z_N|\tau_1,,,\tau_C)=\prod_{u=1}^N \tau_{z_u}\\
%& \pi(\tau_1,,,\tau_C) =\Gamma(\phi C)\Gamma(-\phi^{-C})\prod_{c=1}^C \tau_c^{\phi-1} \quad \text{(dirichlet)}
%\end{align}



%The fact that user u only clicked on a subset of items $\bold{A_u} \in \bold{A}$ with total number of clicks $|c_u|$ indicates that a clicked item is preferred than an unclicked one, i.e. $\bold{S_u(A_u)}=\{R_u \in P_M, s.t. R_{iu}<R_{ku} \text{ if } A_i \in \bold{A_u} \text{ and } A_k \in \bold{A_u^c}\text{ , }\forall i,k,i\neq k\}$
%The sampling can be simplified into 
%\begin{align}
%\begin{split}
%&P(\{\alpha_c,\rho_c\}_{c=1,,,C},z_1,,z_N|\bold{A_1,,A_N})\\
%&=\sum_{R_1 \in \bold{S_1(A_1)}}...\sum_{R_N \in \bold{S_N(A_N)}} P(\{\alpha_c,\rho_c\}_{c=1,,,C},z_1,,z_N, R_1,,,R_N|\bold{A_1,,A_N})
%\end{split}
%\end{align}


\rd 
 Assume now that a given user $u$ has rated $c_u$ items and the objective is to make $k$ recommendations equivalent to inferring items with ranking between $c_u+1$ and $c_u+k$. To find the next top $k$ items for user $u$,  we evaluate the posterior probability 
\begin{equation*}
    P_{iu}=P(c_u+1 <= r_{ui} <= c_u+k|\cdot).
\end{equation*}

The strength of Mallows Model is the use of a distribution of rankings, allowing inference beyond point estimation. The main limitation is the need for computation-expensive posterior MCMC simulation, which is not suitable for large data sets on sequential updating. 

\bk
\rd
\subsection{Generative Models}\bk
In recent years, some papers start to use neural networks or generative models for collaborative filtering (\cite{VCF1},  \cite{cf-bandit}, \cite{NCF}, \cite{VCF2}). Variational Autoencoder is one of the popular methods. \\

\bch The use of variational autoencoder models \ech originated from
% the well-cited Kingma and Welling paper ()
\cite{VAE}. To apply it to the collaborative
filtering, following \cite{VCF2}, we assume the hidden factors are
latent variables $z_u$, the number of clicks of a user to all items is
$x_u=[x_{u1},,,x_{un}]$, $f_\theta(z_u)$ is a non-linear function to
produce a probability distribution of $\pi(z_u)$, and $x_u$ is
multinomial with total number of clicks $N_u$ and probability vector
$\pi(z_u)$.
\begin{align*}
    z_u \sim N(&0,I_k),\quad \pi(z_u)\propto \exp[f_{\theta}(z_u)],\\
    &x_{u} \sim \mathrm{Mult}(N_u, \pi(z_u)),
\end{align*}
One common approach is to use variational inference to approximate the
\cut % true
intractable posterior $p(z_u|x_u)$ with a variational approximate
distribution $q(z_u)$. 
\iffalse
If $q(z_u)$ is set to be fully diagonalized Gaussian 
\begin{equation}
    q(z_u) = N(\mu_u,diag(\sigma_u^2))
\end{equation}
We can see the parameter numbers grows with the number of users and items and can become a bottleneck for large online recommenders. So alternatively, we can use a variational auto-encoder which ‘amortizes’ the cost of inference across datapoints by sharing (amortizing) the variational parameters across datapoints. 

Autoencoders achieve this by replacing individual parameters with a function of data ,i.e, inference model. (Gaussian here is just an example.)
\begin{equation}
    q_{\phi}(z_u|x_u)=N(\mu_{\phi}(x_u),diag\{\sigma^2_{\phi}(x_u)\})
\end{equation}
Minimizing the KL divergence between $q_{\phi}(z_u|x_u)$ and $p_{\theta}(z_u)$ is equivalent to maximizing the ELBO. For each u,
\begin{align}
\begin{split}
    ELBO_u(\theta,\phi)&=\log p(x_u)-KL(q_{\phi}(z_u|x_u)||p(z_u|x_u)) \\
    &=E_{q_{\phi}(z_u|x_u)} [\log p(x_u,z_u)]-E_{q_{\phi}(z_u|x_u)}[\log q_{\phi}(z_u|x_u)]\\
    Or &= E_{q_{\phi}(z_u|x_u)}[\log p(x_u|z_u)]-KL(q_{\phi}(z_u|x_u)||p(z_u))
\end{split}
\end{align}


The optimization of ELBO can be typically done by minibatch stochastic gradient descent, iteratively for $\nabla_{\phi}\frac{N}{M}\sum_{u=1}^M ELBO(x_u)$,$\nabla_{\theta}\frac{N}{M}\sum_{u=1}^M ELBO(x_u)$.
\fi
Full algorithm can be seen in \cite{VCF2} and \cite{VAE}. %Iterate till convergence gives us estimation for $\theta$ and $\phi$, and thus complete inference model of $q_{\phi}(z_u|x_u)$ and the generative model of $p(x_u|z_u)$.

Autorec model (\cite{VCF1}) is another version of this model applied to rating instead of clicking numbers. 

Generative Models with variational inference is an efficient scalable inference well suited when the dataset is large in size and new users' data keep flowing in. The problem is the lack of explanibity, the absence of uncertainty quantification, and the difficulty to fit the model to a more complicated goal, such as a specific criterion for recommendation diversity and accuracy tradeoff. 

\rd need to shorten this and why we are using ours. 
\bk

%\cite{CFRS} (this is the same as 1)
%\cite{ACF} (this is the same as 2)
%\cite{2says10}
%\cite{2says17}
%\cite{2says23} (appear together as 2says 17)
%\cite{PMF} 
%\cite{LDA-like}
%\cite{LDA}
%\cite{cf-bandit} (not sure where it appears)
%\cite{itembased} (not sure where it appears)
%\cite{NCF}
%\cite{VCF1}
%\cite{VCF2}
%\cite{VAE}
%\cite{MM1}
%\cite{MM2}
%\cite{MM3} (this is the same as MM1says7)

%\bibliography{references}




==> model3.tex <==
\section{Double Feature Allocation Model}
\label{sec:model}
\bch We introduce an alternative generative model for user ratings
$r_{ui}$ of users $u=1,\ldots, m$ for items $i=1, \ldots, n$, using
notation as before. We assume ordinal ratings $r_{ui} \in
\{1,\ldots,5\}$. 
The inference \ech  goal is to predict user preferences for \bch un-rated \ech movies by discovering
similarity patterns among users and movies.

A double feature allocation model is a model for random pairs of
subsets, first proposed in \citet{ni2019dfa}. A feature is a subset of
users \bch together with \ech a matching subset of items.  We use
an Indian buffet process 
(IBP) \bch prior to link \ech users and items to features. Suppose
there are $K$ features.
We use an \bch $(m \times K)$ binary matrix $A$ to link users to
features, with $A_{uk}=1$ indicating that user $u$ is in feature
$k$. \ech
Another $(n \times K)$ binary matrix $B$ links items to features,
\bch with $B_{ik}=1$ meaning that movie $i$ is in feature $k$. \ech
\mynote{Q: earlier we used $u$ for users and $i$ for items; best to
  keep it that way, lest we totally consufe our readers..}

We use Table~\ref{tab:illustraion-of-DFA} to illustrate our features. Same colored block indicate one feature $k$, a subset of users and a matching subset of items. 

\begin{table}[]
\begin{tabular}{lllllllll}
         & Item 1                   & Item 2                                          & Item 3                                          & Item 4                                          & Item 5                   & ... & Item n-1 & Item n                   \\
User 1   &                          & {\color[HTML]{333333} }                         & \cellcolor[HTML]{FFCCC9}{\color[HTML]{333333} } & \cellcolor[HTML]{FFCCC9}{\color[HTML]{333333} } & \cellcolor[HTML]{FFCCC9} &     &          &                          \\
User 2   & \cellcolor[HTML]{FFFC9E} & \cellcolor[HTML]{94E9ED}{\color[HTML]{333333} } & \cellcolor[HTML]{94E9ED}{\color[HTML]{333333} } & \cellcolor[HTML]{FFCCC9}{\color[HTML]{333333} } & \cellcolor[HTML]{FFCCC9} &     &          & \cellcolor[HTML]{FFFC9E} \\
User 3   & \cellcolor[HTML]{FFFC9E} & \cellcolor[HTML]{94E9ED}{\color[HTML]{333333} } & \cellcolor[HTML]{94E9ED}{\color[HTML]{333333} } & \cellcolor[HTML]{FFCCC9}{\color[HTML]{333333} } & \cellcolor[HTML]{FFCCC9} &     &          & \cellcolor[HTML]{FFFC9E} \\
User 4   &                          & \cellcolor[HTML]{94E9ED}                        & \cellcolor[HTML]{94E9ED}                        &                                                 &                          &     &          &                          \\
User 5   &                          &                                                 &                                                 &                                                 &                          &     &          &                          \\
...      &                          &                                                 &                                                 &                                                 &                          &     &          &                          \\
User m-1 & \cellcolor[HTML]{FFFC9E} &                                                 &                                                 &                                                 &                          &     &          & \cellcolor[HTML]{FFFC9E} \\
User m   & \cellcolor[HTML]{FFFC9E} &                                                 &                                                 &                                                 &                          &     &          & \cellcolor[HTML]{FFFC9E}
\end{tabular}
\vspace{2mm}
\caption{Illustration of features in Double Feature Allocation Model, with colored box as features.}
\label{tab:illustraion-of-DFA}
\end{table}

\paragraph*{\bch Prior model.}
\mynote{just adding paragraph titles mainly for us to keep track --
  we can drop them eventually again.}
The matrix $A$, the user-feature model, follows an IBP prior 
\citep{griffiths2011indian}.
\bch The model includes an unknown number $K$ of features, and  \ech can be written as
\begin{equation*}
    P(A)=\frac{\lambda^K\text{exp}(-\lambda H)}{K!}\prod_{k=1}^K\frac{\Gamma(m_k)\Gamma(m-m_k+1)}{\Gamma(m+1)},
\end{equation*}
where $\lambda$ is a fixed hyperparameter (concentration parameter), $H$ is the harmonic number $H=\sum_{u=1}^m 1/u$, $m_k$ is the sum of column $k$, $m_{k}=\sum_{u=1}^m A_{uk}$. The number of features $K$ is random and unbounded, and features are exchangeable in order.  

In practice, for the purpose of prior sampling, we only need the conditional probability of $A_{uk}=1$,
\begin{equation*}
    P(A_{uk}=1|A_{-u,k})= m_{-u,k}/m,
\end{equation*}
where $A_{-u,k}$ is the $k$th column of $A$ excluding $A_{uk}$ and $m_{-u,k}$ is the sum of column $k$ of $A$ excluding $A_{uk}$.

\rd The model is best described by a generative definition \cite{griffiths2011indian,broderick2013cluster}. \bk We start from the first row; for each row $i$, the new features numbers $K^+$ are sampled from $\text{Pois}(\lambda/m)$. Suppose current number of nonempty columns are $K$, i.e., current nonempty features are features $1:K$, only in the current row $A_{u,(K+1):(K+K^+)}=1$, in other rows  $A_{-u,(K+1):(K+K^+)}=0$. For $k$ in existing features $1:K$, $p(A_{uk}=1|A_{-u,k})=m_{-u,k}/m$. Section~\ref{sec:posterior-sampling} will explain in detail of posterior sampling of random unbounded $K$ and the $A$ matrix. 

\rd Given $A$, the iterm-feature matrix $B$ inherits $K$ features from $A$. For simplicity, we assume independent Bernoullis: \bk
\begin{equation*}
    P(B_{ik}=1|A)= p,
\end{equation*}
 with the prior parameter $p$ usually chosen to be a small number to control the number of features a movie can be in. Such parsimony ensures that features do not share too many common movies and preserve their differences. In posterior sampling,  $p$ and the dimension of $B$ will be updated each time after we update $A$. 

Note that the IBP $p(A)$ together with $p(B \mid A)$ define a joint model
$p(A,B)$, and therefore also imply a marginal $p(B)$.
\bch The current model does not imply a marginal IBP prior for
$p(B)$. If a more symmetric construction with an IBF marginal prior on $B$ were desired, it could be easily achieved. \ech
Let $p_{IBP}(B)$ denote an IBP prior on a random binary matrix $B$,
including the number of columns, $K_B$, and let 
$p_{IBP}(B \mid K_B)$ denote the conditional distribution of $B$,
conditional on the number of columns equal to $K_B$ under the
IBP. Then using $p(B \mid A) = q(B \mid K_B=K_A)$ would by
construction \bch deliver $p(B)=IBP$, marginally. \ech

\paragraph*{\bch Sampling model.}
Finally, we
\bch complete the inference model with a sampling model for the
observed ratings. The \ech model links features to
ratings
\bch by introducing probabilities for $r_{ui}$ conditional on the
currently imputed features of which user $u$ and movie $i$ are
members. \ech
% That is, given the $i$th user and $j$th movie are in features
% $k^*$, the rating of $R_{ij}$ based on $k^*$.

We consider a baseline $b_0=2.5$ (between the extremes 1 and 5).
Each feature $k$ \bch of which user $u$ and movie $i$ are a member
adds \ech an adjustment $\theta_k$ to this baseline.
For example, feature $k$ \bch might be 
a pair of subsets of comedy movies and comedy fans. Then $\theta_k$
would be a positive increment from baseline. Similarly, if
feature $k$ is a pair of subsets of comedy movies and comedy haters,
then $\theta_k$ should be a negative adjustment. We allow a movie and a
user to be in multiple subsets with features having aggregative
influences. In the same example of comedy movies and comedy fans, if
this user-movies pair also belongs to another subset $k'$,
\bch this would add another increment $\th_{k'}$. \ech

We also include global parameters $\rho_i$ for each movie regardless
of feature allocation. The parameter $\rho_i$ has an
interpretation as overall mean rating for movie $i$ (on the ordinal
probit scale).
\bch This movie-specific offset reflects if \ech
a movie is generally popular and well-received among audiences or vice
versa. 

\bch Specifically, we use \ech
an ordinal probit model including the described feature-specific and
\bch movie-specific parameters. \ech
Denote by  $Z_{ui}$ \bch a latent continuous probit score for the
rating of user $u$ for movie $i$, denote by $K^*_{ui}=\{k:\;
A_{uk}=B_{ki}=1\}$ the set of features that include both, user $u$ and
movie $i$. 
Finally, let \ech $\tau^2$ denote the variance of the latent probit score
$Z_{ui}$.
\bch We use an inverse-gamma hyperprior on $\tau^2$, and normal priors for both
$\theta$ and $\rho$.
We assume \ech
\begin{equation*}
  Z_{ui} \mid
  A,B,\theta,\tau \sim N(b_0+\sum_{k \in K^*}\theta_k+\rho_i,\tau^2).
\end{equation*}
The probit scores are linked with the data in the usual ordinal probit
model as 
\begin{align*}
    r_{ui}= \left\{\begin{array}{cc}
       1,  &  Z_{ui}\leq1\\
       x, x\in\{2,3,4\}, & x-1 < Z_{ui} \leq x\\
       5, &  Z_{ui}>4
    \end{array}\right..
\end{align*}



\section{Posterior Inference}
\label{sec:posterior-sampling}
\subsection{Posterior Sampling Algorithm}
\label{subsec:posterior-algorithm}
\rd We implement posterior inference using MCMC posterior simulation. Let $\omega=(A,B,\theta,\tau,\rho)$ denote the currently computed parameters. See the appendix for transition probabilities to update $B$, $\theta$, $\rho$ and $\tau$. Only the transition probability for $A$ requires more discussion.

Denote the number of iteration as superscript $^{(t)}$, denote $u$th row of $A$ and $R$ as $A_{u\cdot}$,$R_{u\cdot}$, $i$th column of $R$ as $R_{\cdot i}$.
\vspace{5mm}

Transition probability to update $A_{u\cdot}$,
\begin{itemize}
      \item step 1: For all the $k$ with $m_{-u,k} \neq 0$,\\
update $P(A_{uk}=x|\cdot)\propto \frac{m_{-u,k}}{m}p(\rd R_{u\cdot}\bk|A_{uk}=x, A_{-u,k}, \theta,\rho,\tau,B)$, \\ 
$x=\{0,1\}$. 
       \item step 2: Reversible Jump. \\
       Define singular features are features with $m_{-u,k}=0$. At current state $K$ features with $\theta_1,,,\theta_K$,  $K_0$ of them are not singular features, w.l.o.g, note them as $\theta_1,,,\theta_{K_0}$, while $\theta_{K_0+1},,,\theta_{K}$ are singular features. \\
       \begin{itemize}
           \item (2a) For all $k$ in $1:K$, if $m_{-u,k}=0$ , propose $\tilde{A}=A[,-k]$, 
i.e, propose to delete singular features, $K_0+1,,,K$.  Now we only left with $K_0$ fts in proposed $\tilde{A}$ with $\theta_1,,,\theta_{K_0}$ 
          \item (2b) Propose to add in new features, $\tilde{K_u^+}=Pois(K_u^+|\frac{\lambda}{n})$, followed by $\tilde{\theta}_{K_0+1},,,\tilde{\theta}_{K_0+K_u^+} \sim h$, $h$ is the prior for all $\theta$,  add in the new features to $\tilde{A}$, with \\
       $\tilde{A}_{u,K_0+1},\tilde{A}_{u,K_0+2},..., \tilde{A}_{u,K_0+K_i^+}=1$,\\ $\tilde{A}_{-u,K_0+1},\tilde{A}_{-u,K_0+2},..., \tilde{A}_{-u,K_0+K_i^+}=0$ .
       \end{itemize}
       \item 2a and 2b yields a proposal: replacing singular features with new features, i.e. replacing \small{($K_0+1 :K$, $\theta_{K_0+1:K}$)} with ($K_0+1:K_u^+$, $\tilde{\theta}_{K_0+1 :K_u^+}$). This dimension change in proposal requires a reversible jump step with acceptance ratio
       \begin{align*}
       \begin{split}
           \alpha&=\frac{p(R_{u\cdot}|\tilde{A_{u\cdot}},\theta_{1:K_0},\tilde{\theta}_{K_0+1 :K_0+K_u^+})}{p(R_{u\cdot}|Z_u,\theta_{1:K_0},\theta_{K_0+1: K})} \times \frac{h(\tilde{\theta}_{K_0+1 :K_0+K_u^+})Pois(K_u^+|\frac{\lambda}{n})}{h(\theta_{K_0+1 :K})Pois(K-K_0|\frac{\lambda}{n})}\\
           &\times \frac{h(\theta_{K_0+1:K})Pois(K-K_0|\frac{\lambda}{n})}{h(\tilde{\theta}_{K_0+1 :K_0+K_u^+})Pois(K_u^+|\frac{\lambda}{n})}\\
    &=\frac{p(R_{u\cdot}|\tilde{A_{u\cdot}},\theta_{1:K_0},\tilde{\theta}_{K_0+1 :K_0+K_u^+})}{p(R_{u\cdot}|A_{u\cdot},\theta_{1:K_0},\theta_{K_0+1:K})} 
       \end{split}
\end{align*}
With probability $\alpha$ we accept the proposal from 2a 2b. Note that the proposal and prior cancel out each other. \rd Table~\ref{tab:illustration-A-update} illustrate step 2a and 2b procedure. \bk
 
 \bl to appendix  
    \item Update $B^{(t+1)}|R,A^{(t+1)},\mathbf{\theta}^{(t)},\mathbf{\rho}^{(t)},\tau^{(t)}$, \\
    $p(B_{ik}=x|\cdot) \propto p(B_{ik}=x)p(r_{\cdot i}|B_{ik}=x, B_{-i,k},\theta,\rho,\tau, A)$, $x=\{0,1\}$
    
    \item Sample auxiliary variable $\mathbf{Z}|R,A^{(t+1)},B^{(t+1)},\mathbf{\theta}^{(t)},\mathbf{\rho}^{(t)},\tau^{(t)}$
    $$p(Z_{ui}|\cdot) \sim \mathrm{TruncatedNormal}(b_0+\sum_{k \in K^*}\theta_k+\rho_i,\tau^2) $$
    with lower bound $r_{ui}-1$ \rd($r_{ui}>0$)\bk,  upper bound $r_{ui}$ \rd($r_{ui}\leq 5$)\bk, $K^*$ is the set of $k$ where $A_{uk}=B_{ik}=1$.
    
    \item Update $\mathbf{\tau}^{(t+1)}|\mathbf{Z},A^{(t+1)},B^{(t+1)},\mathbf{\theta}^{(t+1)},\mathbf{\rho}^{(t+1)}$ from conjuagate Inverse-Gamma families.
    \rd
    \item Update $\mathbf{\theta}^{(t+1)}|\mathbf{\rho}^{(t+1)},\mathbf{Z},\tau^{(t)},A^{(t+1)},B^{(t+1)}$ and $\mathbf{\rho}^{(t+1)}|\mathbf{\theta}^{(t+1)},\mathbf{Z},\tau^{(t)},A^{(t+1)},B^{(t+1)}$ from conjuagate Normal families. 
    \bk
\end{itemize}
\bk
We predict unseen ratings by maximizing the posterior predictive probability,
\begin{equation}
  \hat{r}_{ui}=  \argmax_{x\in \{1,2,3,4,5\}} \int p(R_{ui}^{mis}=x|A,B,\theta,\tau,\rho) p(A,B,\theta,\tau,\rho|R^{obs})dw.
\end{equation}


\begin{table}[]
\begin{tabular}{lllllllllll}
       & Ft1 & Ft2 & ... & Ft $K_0$ & Ft $K_0+1$                 & ...                       & Ft $K$                       & Ft $K_0+1$ '                & ...                       & Ft $K_0+ K_u^+$           \\
User 1 & 1  & 1  &     & 0      & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 \\
User 2 & 1  & 1  &     & 1      & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 \\
...    & 1  & 0  &     & 1      & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 \\
User u & 1  & 1  &     & 0      & \cellcolor[HTML]{68CBD0}1 & \cellcolor[HTML]{68CBD0}1 & \cellcolor[HTML]{68CBD0}1 & \cellcolor[HTML]{FFCE93}1 & \cellcolor[HTML]{FFCE93}1 & \cellcolor[HTML]{FFCE93}1 \\
...    &    &    &     &        & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 \\
User m & 1  & 1  &     & 1      & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{68CBD0}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0 & \cellcolor[HTML]{FFCE93}0
\end{tabular}
\caption{Illustration of Feature Swap in Posterior Matrix A Update. Step 2 propose to delete blue columns and add in orange columns. }
\label{tab: illustration-A-update}
\end{table}


\subsection{A Consensus Monte Carlo Method for Large Number of Users}
\label{subsec:concensus-monte-carlo}

The described posterior simulation can be computationally costly. %The running time would increase in O()
Large recommender systems usually have at least thousands, or millions of users, render the usual MCMC impractical. Thus we use the idea of Consensus Monte Carlo \citep{scott2016bayes-consensus},  to  split data into shards, run MCMC one each shard in parallel on different machines, and then \rd reconcile posterior inference from the shards into a reconstruction of posterior inference under the full data.  \citet{ni2019consensus} applied Consensus Monte Carlo to Bayesian nonparametric models on clustering and feature allocation. Their method relies on shared data points (anchor points) across shards, and they merge random subsets (clusters or features) on different machines based on the number of common anchor points in the two sets. This strategy, though appealing, does not work in our case. \newcommand{\rhot}{\tilde\rho}
\newcommand{\sig}{\sigma}

Using a set of users as common anchors to define a criterion for
merging features would ignore the possibility of different sets of
movies being paired with these users in different shards. 
And similarly for using sets of movies only. A practicable
implementation would need to use a criterion based on shared users,
shared movies and similar imputed feature-specific effects $\th_k$.
A related criterion to merge subsets would require several ad-hoc choices and tuning parameters. In simulations we found that the involved approximations left the joint posterior reconstruction of little practical value. Instead we propose an alternative strategy based on CMC for global parameters, but keeping inference for random subsets local to each shard. We refer to this strategy as "semi-local CMC".

We use shards that split the data by subsets of users. 
Let $s=1, \ldots, S$ index the shards, and let $\bigcup_{s=1}^S U_i =
\{1, \ldots, m\}$ denote the split of users into the $S$ shards.
Also, let $R_s$ denote the data for the users in shard $s$.
In our model, the random features that are imputed under posterior
inference under shard $s$ naturally include only users from $U_s$,
making the features local parameters, while the only global
parameters are $\rho_i, i=1, \ldots, n$.
% Let $\omega=(A,B,\rho,\tau)$ denote the unknown parameters, and let
% $p_s(\omega \mid R_s)$ denote the shard-specific posterior
% distributions.
We use a CMC approximation of the joint posterior for the global
parameter $\rho$ as
$$
   p(\rho \mid R) \approx \prod_{s=1}^s p(R_s \mid \rho)\,
   p(\rho)^{1/S}.
$$
The nature of the approximation is to assume independence of the
marginal distribution of global parameters across shards. 
Conditional on a posterior sample $\rhot \sim p(\rho \mid R)$ we then
user shard-specific posterior samples conditional on $\rhot$. The
latter is implemented by selecting stored posterior Monte Carlo samples $(A,B,\theta,\rho,\tau)$ with $|\rho-\tilde{\rho}|<\epsilon$.
Here $A$ refers to users in shard $s$ only, and $B$ and $\theta$ are
linked with the subsets that are represented by $A$, making
$(A,B,\theta)$ parameters that are local to each shard only.

There remains the step of creating a Monte Carlo sample for
$\rho \sim p(\rho \mid R)$. For this we use CMC for approximate normal
posterior distributions. Let $(\mu_s, \sigma_s)$ denote posterior mean
and standard deviation of $\rho_i$ in shard $s$ (for a movie $i$).
We approximate $p(\rho \mid R) \approx N(\mu, \sig)$ with
$1/\sig^2 = 1/\sig^2_0 + \sum_s 1/\sig^2_s$ and $\mu_s = \ldots$,
where $(\mu_0, \sig^2_0)$ are the prior moments for $\rho$.
We refer to the strategy as semi-local CMC.
\iffalse
\bl The subsets (features) of pairs of movies and users depend very much on the neighbours in shards. Furthermore, if two subsets are merging owing to number of shard anchors (users in this case), it is not necessarily the two subsets should have similar $\theta$; these users could be comedy lovers and romantic haters at the same time. \bk One step forward, in the case of two subsets share similar users and movies, since the ratings are ordinal data, it is not clear how to define a criterion of merging and how to merge $\theta$ in a way to preserve the transitivity. 

Thus, we need a new technique to perform consensus monte carlo in our case. Instead of letting shards share users as anchors, we let each shards share global variables. We split shards on users but keep entire movie collections. The movie-specific $\rho$ are shared across shards as a global variable. We thus follow the original idea of \citet{scott2016bayes-consensus}. Suppose there are $S$ shards, 
\begin{equation*}
    p(\rho |R)\propto \prod_{s=1}^S p(R_s|\rho)p(\rho)^{1/S}
\end{equation*}
where $p(R_s|\rho)$ and $p(\rho)$ are both normal, each shard is equally weighted, then we have
\begin{equation*}
    p(\rho|R)\sim N(\overline{\mu_s},\frac{1}{1/\sigma_0^2+\sum_sn_s/\sigma_s^2}),
\end{equation*}
where $\mu_s$, $\sigma^2_s$ are shard-specific posterior parameters in $\rho_s|R_s \sim N(\mu_s, \sigma_s^2)$, and $\mu_0$, $S\sigma_0^2$ are prior parameters of in each shard $\rho \sim N(\mu_0,S\sigma^2_0)$, suppose $\sigma_0>>\sigma_s$ such that $\mu_s\approx \overline{R_s}$, and $n_s$ the number of users in each shard is the same.
\fi

\bl
\mynote{should I keep this below?}
The full algorithm is now, run MCMC described in Section~\ref{subsec:posterior-algorithm} on each separate shards, store $A$, $B$, $\theta$, $\tau$, $\rho$, every 5 iterations. Merging $\rho$ across shards as above yields a global posterior $\tilde{\rho}$. In each shard, for each stored iteration $A$, $B$, $\theta$, $\tau$, resample $\tilde{\rho}$ from the global distributions, filter the iterations where the stored shard-posterior $\rho$ is close to resampled global $\tilde{\rho}$ and make predictions based on $A$, $B$, $\theta$, $\tau$ and $\tilde{\rho}$ in these iterations. Note that the filtering step within the shard is to ensure the closeness of shard posterior MCMC and global posterior MCMC and to not totally lose the dependence of $\tilde{\rho}$ and $(A,B,\theta,\tau)$ in the iterations we use for prediction. 

\vspace{5mm}

Algorithm 2: CMC
\begin{itemize}
    \item Separate users into S shards, keep entire list of movies. 
    \item In each shard, do Alrogrithm 1: MCMC. Store $A$, $B$, $\mathbf{\theta}$, $\mathbf{\tau}$, $\mathbf{\rho}$ every 5 iterations. 
    \item Merge $\rho$ from each shard: calculate the global posterior distribution of $\mathbf{\rho}$ by aggregating shard precision. 
    \item In each shard, for each stored iteration, resampling $\mathbf{\tilde{\rho}}$ from global posterior, keep those iterations where $|\rho-\tilde{\rho}|<\epsilon$, perform prediction by  $A$, $B$, $\mathbf{\theta}$, $\mathbf{\tau}$ and resampled $\tilde{\rho}$ in those iterations. 
\end{itemize}
\bk

\iffalse
\begin{figure}
\vspace{-5mm}
    \centering
    \includegraphics[width=0.6\textwidth]{plots/illustration-CMC.png}
    \vspace{-2mm}
    \caption{Illustration of Concencus Monte Carlo and merging $\rho$.}
    \label{fig:pair-comp}
\end{figure}
\fi


==> result3.tex <==
\section{Preference Predicion with MovieLens Data}
\label{sec:experiment}
We use the Movielens dataset \footnote{https://grouplens.org/datasets/} with movie ratings from 6040 users.  We clean the data in the same way described in \citet{MM3} to make our model result comparable.  We keep $200$ most rated movies and users who rated more than three movies, which yields to a $6040\times 200$ rating matrix $R$. Our goal is to predict the preference of unseen movies to rated movies for each user. Here preference is defined as the following. Denote preference relation as $\succ$. Denote predicted rating of user $u$ for movie $i$ is $\hat{R}_{ui}$, estimated from Section\ref{sec:model}. We say user $u$ strictly prefers movie $i$ to $i'$, ($i \succ i'$ for user $u$), if $\hat{R}_{ui}$ is strictly higher than $\hat{R}_{ui'}$. 

In the $6040\times 200$ rating matrix, only $24.7\%$ entries are observed. We conduct a pairwise preference prediction test using our model. For each user, we randomly select one movie he/she has rated as test, and train the rest observed ratings. We compare this user's the preference of this test movie to other rated movie by comparing the test predicted rating to training predicted rating. This pairwise preference test is also comparable to \citet{MM3}.

We apply a double IBP prior described in Section~\ref{sec:model} initialized with $\lambda=3$, base line $\theta=2.5$, non-baseline $\theta$s drawn from $N(0,\sigma_0^2)$,  $\sigma_0=2$, $\tau$ drawn from an inverse-gamma distribution with location and scale parameters $(5,1)$.  We initialize the number of features $K$ from matrix factorization algorithm for recommender system from \cite{funk2006MF}. 

Following the posterior sampling scheme with Concensus Monte Carlo in Algorithm 2, we divided $6040$ users into $15$ shards and run shards' MCMC as Algorithm 1 in parallel. 
Each shard with $400$ users and $200$ movies stabilizes at around $38$ to $42$ features. %We merge the shards global variable $\rho$ and re-predict each rating in each shard using re-sampled $\rho$ from merged posterior. 
As we described in Section~\ref{sec:posterior-sampling}, we merge shards by merging global variable $\rho$. The after-merge prediction follows from re-sampling $\rho$ from global posterior and previously stored MCMC draws of other variables.

The resulting average pairwise preference accuracy in each shard is $79.1\%$ with standard deviation $0.012$. \cite{MM3} pairwise comparison on the same data has accuracy of $79.6\%$. 

Figure~\ref{fig:pair-comp} shows the before-merge individual shards MCMC pairwise predication accuracy and after-merge pairwise predication accuracy. After-merge prediction accuracy has a higher average and a smaller standard deviation among shards.

\begin{figure}
\vspace{-5mm}
    \centering
    \includegraphics[width=0.8\textwidth,height=0.6\textwidth]{plots/pair-comp-newmerge.pdf}
    \vspace{-5mm}
    \caption{Pairwise Comparison Prediction Accuracy in each shard before and after merge}
    \label{fig:pair-comp}
\end{figure}

For exact predicted rating for unseen movies, on the test set within one star distance, our model has provided $88.5\%$ accuracy. That is saying, we have on average $88.5\%$ probability that our predicted rating is at or within in one star difference of the actual rating.  %  That is saying, we have on average $88.5\%$ probability that we predict the ratings at the actual ratings within one star difference. 
Figure 2 shows in each shard the prediction accuracy and its $95\%$ Confidence Interval using binomial distribution variance and a normal approximation CI, $(\hat{p}- \mathit{z}_{\alpha} \sqrt{\frac{\hat{p}(1-\hat{p})}{n_s}},\hat{p}+ \mathit{z}_{\alpha} \sqrt{\frac{\hat{p}(1-\hat{p})}{n_s},}$,where $\hat{p}$ denotes the shard accuracy,   $\mathit{z}_{\alpha}$ denotes $1-\frac{\alpha}{2}$ quantile of a standard normal distribution, $\alpha=0.05$.

\begin{figure}
\vspace{-5mm}
    \centering
    \includegraphics[width=0.8\textwidth,height=0.6\textwidth]{plots/pred-acc.pdf}
    \vspace{-5mm}
    \caption{Accuracy of predicting unseen movies within one star distance in each shard after merge and their $95\%$ confidence intervals. Red line indicates the mean over shards.}
    \label{fig:pair-comp}
\end{figure}


Here we also present the computational complexity reduction from our consensus monte carlo method. \cite{ghahramani2006infinite} has established that an indian buffet process with $N$ data points with linear-Gaussian likelihood model with at least have $O(N^3)$ computation complexity per iteration. To be specific, \cite{doshi2009accelerated} pointed out that in each iteration for $N$ $D$-dimensional data points and a linear-Gaussian likelihood model, given an $N\times K$ feature assignment matrix in that iteration, the collapsed Gibbs sampler has complexity $O(N^3(K^2+KD))$. In our double feature allocation model with 
$m\times K$ matrix $A$ and $n\times K$ matrix $B$ ($m>n$) and a probit likelihood model will at least have complexity $O(m^3)$ each iteration. If we break the entire data set into $S$ shards then we will have complexity of $S\times O((m/S)^3)$ each iteration. With $m=6000$ in Movielens data, we see in Figure ~\ref{fig:comp-sd} the complexity per iteration decreases and eventually stabilizes with $S$. We also note that more shards would result in fewer users in a shard and thus fewer ratings observed in each feature in the shard and a larger standard error of feature associated parameter $\theta$. Consider the normal distribution of $\theta$, heuristically the standard error of $\theta_k$ would be proportional to $\frac{\tau^2}{n_{ks}}$ where $n_{ks}$ is the number of ratings observed in feature $k$ in the shard $s$. Suppose coarsely the number of ratings observed in the feature in a shard is proportional to the number of users and number of movies in the shard and inversely proportional to number of features in shard $s$, $n_{ks} \propto m_s\times n/\log(m_s\times n)$, $\log(m_s\times n)$ being the approximate number of clusters in shard $s$ \rd \citep{korwar1973contributions}
\bk. Then standard of error of $\theta_k$ is proportional to $1/\sqrt{m_s\times n)/\log(m_s\times n)}$. Figure \ref{fig:comp-sd} shows this trade-off of standard error of estimating $\theta_k$ increasing with number of shards $S$ while the computation cost per iteration decreasing with $S$. 

%\rd
%maybe instead of $sd_\theta$ I should talk about random sampling error? it's also going to be an increasing line.
%\bk

\begin{figure}
\vspace{-5mm}
    \centering
    \includegraphics[width=0.75\textwidth]{plots/comp-sd.png}
    \vspace{-3mm}
    \caption{Complexity per iteration and standard error of $\theta$ with the number of shards in consensus monte carlo, $\propto$ denotes proportional up to a constant.}
    \label{fig:comp-sd}
\end{figure}



